Enhancing Data-Awareness of Object-Centric Event Logs

When multiple objects are involved in a process, there is an opportunity for processes to be discovered from different angles with new information that previously might not have been analyzed from a single object point of view. This does require that all the information of event/object attributes and their values are stored within logs including attributes that have a list of values or attributes with values that change over time. It also requires that attributes can unambiguously be linked to an object, an event or both. As such, object-centric event logs are an interesting development in process mining as they support the presence of multiple types of objects. First, this paper shows that the current object-centric event log formats do not support the aforementioned aspects to their full potential since the possibility to support dynamic object attributes (attributes with changing values) is not supported by existing formats. Next, this paper introduces a novel enriched object-centric event log format tackling the aforementioned issues alongside an algorithm that automatically translates XES logs to this Data-aware OCEL (DOCEL) format.

==> float/README <==

  The float package
  =================

This package improves the interface for defining floating objects such
as figures and tables in LaTeX.  It adds the notion of a `float style'
that governs appearance of floats.  New kinds of floats may be defined
using a \newfloat command analogous to \newtheorem.  This style option
also incorporates the functionality of David Carlisle's style option
`here', giving floating environments a [H] option which means `PUT IT
HERE' (as opposed to the standard [h] option which means `You may put
it here if you like').

Run `float.ins' through LaTeX to produce float.sty from float.dtx.
Run `float.dtx' through LaTeX to produce the documentation.

This program can be redistributed and/or modified under the terms
of the LaTeX Project Public License distributed from CTAN archives
in the directory macros/latex/base/lppl.txt; either version 1 of
the License, or (at your option) any later version.

                                Anselm Lingnau <anselm@strathspey.org>


==> hyperref/abbr.tex <==
\abbrdef{``}{\texorpdfstring{``}{\flqq}}
\abbrdef{''}{\texorpdfstring{''}{\frqq}}
\abbrdef{acroread}{\Program{AcrobatReader}}
\abbrdef{aux}{\File{.aux}}
\abbrdef{eg}{e.\,g\mbox{.}}
\abbrdef{gdi}{general document information}
\abbrdef{gs}{\Program{ghost\-script}}
\abbrdef{hyperref}{\Package{hy\-per\-ref}}
\abbrdef{hypbmsec}{\Package{hypbmsec}}
\abbrdef{ind}{\hbox{\texttt{ \ }}}
\abbrdef{isolatin1}{ISOLatin1}
\abbrdef{latex}{\LaTeX}
\abbrdef{latexe}{\texorpdfstring{\LaTeXe}{LaTeX2e}}
\abbrdef{mediabox}{/MediaBox}
\abbrdef{PD1}{PD1}
\abbrdef{pdf}{PDF}
\abbrdef{pdfdocencoding}{PDFDocEncoding}
\abbrdef{pdffile}{pdf file}
\abbrdef{pdfinfo}{\Program{pdfinfo}}
\abbrdef{pdfspec}{*pdf* specification}
\abbrdef{pdfstringdef}{\cms{pdfstringdef}}
\abbrdef{pdftex}{\Program{\pdfTeX}}
\abbrdef{perlscript}{perl script}
\abbrdef{plain}{plain}
\abbrdef{plaintex}{*plain*-*tex*}
\abbrdef{postscript}{PostScript}
\abbrdef{PU}{PU}
\abbrdef{sectioning}{section} % section?
\abbrdef{Sectioning}{Section}
\abbrdef{tex}{\TeX}
\abbrdef{texfile}{*tex* file}
\abbrdef{thumbpdf}{\Package{thumb\-pdf}}
\abbrdef{thumbpdf.pl}{\File{thumbpdf.pl}}
\abbrdef{toc}{\File{.toc}}
\abbrdef{unicode}{Unicode}
\abbrdef{winansiencoding}{WinAnsiEncoding}
\endinput


==> hyperref/docinfo.tex <==
\foilhead[-\baselineskip]{General Document Information}

%\begin{Nav}{\NavInfo\NavBack}%
\begin{Nav}{\NavInfo}%
  \newcommand{\tit}[1]{%
    \multicolumn{2}{@{}l@{}}{\textbf{#1}}\\[0.5ex]%
  }
  \newcommand{\longentry}[1]{%
    \multicolumn{2}{@{}l@{}}{#1}%
  }
  \noindent
  Application: search engines.

  \noindent
  \begin{minipage}[t]{.55\linewidth}
    \begin{tabular}[t]{@{}l>{\tt}l@{}}
    \tit{\hypertarget{info}{*hyperref* options:}}%
    Title:&\Blue{pdftitle}\\
    Subject:&\Blue{pdfsubject}\\
    Author:&\Blue{pdfauthor}\\
    Keywords:&\Blue{pdfkeywords}\\
    Creator:&\Blue{pdfcreator}\\
    Producer:&\Blue{pdfproducer}
    \end{tabular}
  \end{minipage}%
  \begin{minipage}[t]{.45\linewidth}
    \begin{tabular}[t]{@{}ll@{}}
      \tit{Times:}%
      Created:&\Green{/CreationDate}\\
      Modificated:&\Green{/ModDate}\\[1ex]
      \tit{Informations:}%
      \longentry{File name, file size}\\
      \longentry{*pdf* version}\\
      \longentry{Optimized(linearized)}
    \end{tabular}
  \end{minipage}

  \subfoilhead{Setting\texorpdfstring{ the general document information}{}}
  \begin{smallpar}\hypertarget{infoanw}{}%
  \noindent
  \Code{\cms{usepackage}\{hyperref\}}\par
  \vspace{-\parskip}
  \catcode`\^^M=5
  \verbatiminput{pdfinfo}
  \end{smallpar}
  \newpage

\end{Nav}


\iffalse
\begingroup
  \makeatletter
  \def\hyper@anchorstart#1\hyper@anchorend{}%
  \pdfbookmark[1]{\file{hyperref} options}{optinfo}
\endgroup
\fi

\endinput


==> hyperref/encoding.tex <==
\clearpage
\pdfbookmark[0]{Encodings}{enc}

\begingroup
\hypersetup{bookmarksopenlevel=2}


\subfoilhead[-\baselineskip]{Font encoding mechanism%
  \texorpdfstring{}{ of \abbr{latexe}}}

\noindent
\begin{tabular}{@{}l@{ }l@{ $\Rightarrow$ }l@{}}
plain-\TeX:& \code[green]<\ss>\ = \code[blue]<\char"19>&\Red{\ss}\\[1ex]
\LaTeXe:
  & \code<\fontencoding{OT1}\selectfont\char"19>&\Red{\ss}\\
  & \code<\fontencoding {T1}\selectfont\char"19>&\Red{\i}\\[0.5ex]
  & \code<\ss>\ = \code[blue]<\OT1-cmd \ss > \code[green]<\OT1\ss>&\Red{\ss}
\end{tabular}

\noindent
The font slot positions depend on the encoding:\\
\phantom{plain-\TeX: }\code[green]<\OT1\ss>\ = \code<\char"19>\\
\phantom{plain-\TeX: }\code[green]<\T1\ss>\phantom{\code<O>} =
  \code<\char"FF>\\
\phantom{plain-\TeX: }\code[green]<\?\ss>\phantom{\code<OT>} =
  \code<\UseTextSymbol{OT1}\ss>

%\begin{smallpar}
  \noindent
  \code<\> \code[blue]<OT1\ss>\ =
  \code<\csname > \code[blue]<OT1> \code<\string> \code[blue]<\ss>
    \code<\endcsname>
%\end{smallpar}


\subfoilhead[-\baselineskip]{PD1 encoding%
  \texorpdfstring{ (\abbr{pdfdocencoding})}{}}

\begin{itemize}
\def\1{\code[red]}%
\def\2{\code[blue]}\def\3{\Blue}%
\def\4#1{\Green{#1}\,=\,}%
\def\5{\Green}
\item Most names: \1<\text>%
    \3{\textsl{\textless glyph name\textgreater}}\\
    Examples:\quad
  \begin{tabular}[t]{@{}c@{\,=\,}l@{,\quad}c@{\,=\,}l@{}}
    \5\textregistered&\1<\text>\2<registered>&
    \5\textasciitilde&\1<\text>\2<asciitilde>
  \end{tabular}
\item Traditional *tex* and *latex* names.\\
    Examples:\quad
    \4\AE\2<\AE>,\quad
    \4\ss\2<\ss>
\item Accented characters.\\
    Examples:\quad
    \4{\"U}\2<\"U>,\quad
    \4{\c c}\2<\c c>,\quad
    \4{\r A}\2<\r A>~($\Leftarrow$\,\1<\AA>)
\item Escape octal sequences are the result:
%  \2<\textmu>\ (\Green{$\mu$}) $\Rightarrow$ \1<\265>
%  \2<\guillemotleft>\ (\Green{\guillemotleft}) $\Rightarrow$ \1<\253>
  \2<\textmu>\,$\Rightarrow$\,\1<\265>
\end{itemize}


\subfoilhead[-1.5\baselineskip]{PU encoding%
  \texorpdfstring{ (\abbr{unicode})}{}}

\begin{itemize}
\item[\frownie] Characters having catcodes 11 (letter) and 12 (other):\\
Checking each token, high memory and time consumption.
\item[\frownie] Ligatures: same as above.
\item[\frownie] Direct commands:\\
  Easier to implement, but each command must be redefined each time.
\item[\smiley] Commands of *latexe*'s fontencoding mechanism:\\
  Smallest memory consumption and fastest method.\\
  This method is used by package *hyperref*.
\end{itemize}


\subsubfoilhead[-\baselineskip]{Examples of \abbr{unicode} bookmarks}

\begingroup
\def\top#1{\vtop{\vskip0pt\hbox{#1}}}
\def\use#1{\top{\includegraphics[scale=1.2]{u0#1}}}
\centering
\begin{tabular}{@{}ll@{}}
\Blue{Greek}:&\Blue{Cyrillic}:\\
\use{3}&\use{4}\\
\end{tabular}
\par
\endgroup

\endgroup
\endinput


==> hyperref/ende.tex <==
\clearpage
\pdfbookmark[0]{Ende}{ende}

\subfoilhead[-1.5\baselineskip]{Zusammenfassung}
\begin{itemize}
  \item \Red{Dokumenteninformation}:
    \begin{itemize}
      \item \file{hyperref}-Optionen in \code[blue]<\hypersetup>.
    \end{itemize}
  \item \Red{Lesezeichen}:
    \begin{itemize}
      \item Vorsicht wegen fehlender Magenverarbeitung
      \item Vieles durch \code[blue]<hyperref.sty>\ automatisiert.
      \item Zusatzpaket \code[blue]<hypbmsec.sty>
      \item Besondere Effekte erfordern "`low level"'-Eingriffe.
    \end{itemize}
  \item \Red{Thumbnails}:
    \begin{itemize}
      \item
      Einfache Benutzerschnittstelle mit \code[blue]<thumbpdf>.
    \end{itemize}
\end{itemize}


\subfoilhead[-\baselineskip]{Bezugsquellen}

\begin{smallpar}
\pdfadjustspacing=1
\noindent
\begingroup
\def\it{\textbullet}%
\def\sep{1ex}%
\begin{tabularx}{\linewidth}{@{}l@{ }X@{}}
  \it&\Blue{PDF-Spezifikation}:\hfill
\url{http://www.adobe.com/supportservice/devrelations/PDFS/TN/PDFSPEC.PDF}\\[\sep]
  \it&\Blue{pdf\TeX}: \url{http://www.tug.org/applications/pdftex/}\\
  &Win32: \url{ftp://ftp.ese-metz.fr/pub/TeX/win32-beta/}\\
  &Dokumantation: \url{http://www.pragma-ade.nl/pdftex.htm}\\[\sep]
  \it&\Blue{hyperref}, \Blue{pd1enc.def}, \Blue{hyparen.sty}:
\url{ftp://ftp.dante.de/tex-archive/macros/latex/contrib/supported/hyperref/}\\[\sep]
  \it&\Blue{hypbmsec}: Noch per E-Mail, CTAN geplant.\\[\sep]
  \it&\Blue{thumbpdf}:\hfill
\url{ftp://ftp.dante.de/tex-archive/macros/pdftex/thumbpdf/}\\[\sep]
  \it&\Blue{ghostscript}:
\url{http://www.cs.wisc.edu/~ghost/} oder\\&
\url{http://ftp.dante.de/tex-archive/support/ghostscript/aladdin/}
\end{tabularx}
\endgroup
\end{smallpar}

\rightfooter{%
  \ifprint
  \else
    \NavFull\NavSep\NavPrev\NavSep\NavQuit
  \fi
}


==> hyperref/eurobm99.tex <==
%\includeonly{title,docinfo,strings,encoding,psd,hyperref,replace,pdfextra,thumb,summary,links,appendix}
%\includeonly{hyperref}

\begin{document}
\catcode`\*=\active
\include{title}
\include{docinfo}
\include{strings}
\include{encoding}
\include{psd}
\include{hyperref}
\include{replace}
\include{pdfextra}
\include{thumb}
\include{summary}
\include{links}
\include{appendix}
\end{document}


==> hyperref/hyperref.tex <==
\foilhead{Bookmarks with package *hyperref*}
\begin{itemize}
\item Places for options.
\item Options for bookmarks.
\item Creating bookmarks.
\item Replacement methods.
\end{itemize}

\begingroup
\hypersetup{bookmarksopenlevel=2}

\subfoilhead{Places for \texorpdfstring{*hyperref* }{}options}
\begin{enumerate}
\item Global: \Blue{\cms{documentclass}}\Code{[}\dots\Code{]} (*eg* driver)
\item Package: \Blue{\cms{usepackage}}\Code{[}\dots\Code{]}
\item Configuration file: \Blue{\File{hyperref.cfg}} with \cms{hypersetup}
\item After package has been loaded:
  \Blue{\cms{hypersetup}}\Code{\{}\dots\Code{\}}\\
  (*eg* *pdf* information options)
\end{enumerate}


\subfoilhead[-1.5\baselineskip]{Bookmark options}

\begingroup
  \def\sep{0.5ex}
  \noindent
  \Red{\Option{bookmarks}}: Make bookmarks
    (default: \Green{\Value{true}}).\\[\sep]
  \Red{\Option{bookmarksnumbered}}: Put section numbers in bookmarks
    (\Green{\Value{false}}).\\[\sep]
  \Red{\Option{bookmarksopen}}: Open up bookmark tree
     (default: \Green{\Value{false}}).\\[\sep]
  \Red{\Option{bookmarksopenlevel}}: Level, to which bookmarks are
     open.\\[\sep]
  \Red{\Option{pdfpagemode}}: How document starts when opened
     (default: \Green{\Value{None}}):
  \begingroup
    \mbox\qquad\Blue{\Option{None}}: Neither outlines nor thumbnails are visible.\\
    \mbox\qquad\Blue{\Option{UseOutlines}}, \Blue{\Option{UseThumbs}}:
      Outlines, thumbnails are visible.\\
    \mbox\qquad\Blue{\Option{FullScreen}}: Full-screen mode.\\[\sep]
  \endgroup
  \Red{\Option{unicode}}: Bookmarks in *unicode*
     (\Green{\Value{false}}). After package has been\\
     \mbox\qquad loaded, it switches between *unicode* and *pdfdocencoding*.
\endgroup


\subfoilhead[-0.5\baselineskip]{%
  \texorpdfstring{Bookmarks by \abbr{sectioning}}{\abbr{Sectioning}} %
  commands
}
\label{sec:bmbysec}

\begin{itemize}
\item Automatically addition of bookmarks by:
      \begin{itemize}
      \item \cms{part}, \cms{chapter}, \cms{section}, \cms{subsection}, \dots
      \item \cms{addcontentsline}
      \end{itemize}
\item Help file \Blue{\Code{\textsl{\cms{jobname}}.out}}:
      \begin{itemize}
      \item It is written in the \Green{first} run.
      \item The bookmarks are set in the \Green{second} run.
      \item There is \Green{\emph{no}} ``rerun'' warning.
      \end{itemize}
\end{itemize}


\subfoilhead{Tree structure\texorpdfstring{ of bookmarks}{}}

\begin{itemize}
\item Subentries must be added to \Blue{direct} ancestores,
      \Blue{not} grandparents.
\item If an intermediate level is omitted, the leaf starts \Blue{leftmost}:
      \begin{quote}
        \def\sub{\Red{\ensuremath{\rightarrow}}}%
        \def\ver{\Red{\ensuremath{\|}}}%
        \begin{tabular}{@{}lll@{}}
        &\Blue{table of contents}&\Blue{bookmarks}\\
        \hline
        \cms{part}\Code{\{I\}}&\ver{Part I}&\ver{main entry}\\
        \cms{chapter}\Code{\{5\}}&%
          \ver\sub{Chapter I.5}&\ver\sub{subentry}\\
        \cms{subsection}\Code{\{1\}}&
          \ver\sub\sub\sub{Subsection I.5.0.1}&\ver{main entry}\\
        \end{tabular}
      \end{quote}
\end{itemize}


\subfoilhead[-\baselineskip]{\texorpdfstring{Creating bookmarks with }{}\cms{pdfbookmark}}

\begin{itemize}
\item The bookmarks of *sectioning* commands have an \Red{level} number:
      \par\noindent
      \begin{tabular}{@{}lc@{ }c@{ }c@{ }c@{ }c@{}}
      documentclass&\cms{part}&\cms{chapter}&%
        \cms{section}&\cms{subsection}&\dots\\
      \Class{book}/\Class{report}:&\Red{\llap{$-$}1}&%
        \Red0&\Red1&\Red2&\dots\\
      \Class{article}:&\Red0&&\Red1&\Red2&\dots\\
      \end{tabular}
\item Syntax of \Blue{\cms{pdfbookmark}} (default for level: \Red{0}):
      \begin{quote}
        \Blue{\cms{pdfbookmark}}%
          \Code{[\Red{\emph{level}}]\{\emph{bookmark text}\}%
            \{\Green{\emph{anchor name}}\}}
      \end{quote}
\item \Blue{\cms{currentpdfbookmark}}%
        \Code{\{\emph{bookmark}\}\{\Green{\emph{anchor}}\}}%
        \commentchar\ \Red{current level}
\item \Blue{\cms{subpdfbookmark}}%
        \Code{\{\emph{bookmark}\}\{\Green{\emph{anchor}}\}}%
        \commentchar\ \Red{current level + 1}
\end{itemize}


\subsubfoilhead[-\baselineskip]{Using anchors%
  \texorpdfstring{ with \cms{pdfbookmark}}{}%
}

\begin{itemize}
\item An \Green{anchor name} consists of the argument and
      the level:
      \begin{quote}
        \Blue{\cms{pdfbookmark}}\Code{[\Red0]\{Titlepage\}\{\Green{tit}\}}%
          \Code{\commentchar\ }anchor: \Code{\Green{tit}.\Red0}
      \end{quote}
\item The bookmark can point to another \Green{target} (\Green{anchor}):
      \begin{quote}\small
        \cms{hypertarget}\Code{\{\Green{place.}\Red{1}\}\{\}}
      \end{quote}
      Redirecting the bookmark to the previous defined \Green{target}:
      \begin{quote}\small
        \cms{begingroup}\\
        *ind*\cms{makeatletter}\\
        *ind*\cms{def}\cms{hyper@anchorstart}\Code{ \#1}%
          \cms{hyper@anchorend}\Code{\{\}\%}\\
        *ind*\Blue{\cms{pdfbookmark}}\Code{[\Red1]\{Go to the place\}\{\Green{place}\}\%}\\
        \cms{endgroup}
      \end{quote}
\end{itemize}

\endgroup
\endinput


==> hyperref/links.tex <==
\subfoilhead[-\baselineskip]{Links}

\begin{Nav}{\NavBookmarks\NavQuit}

\begin{smallpar}
\let\Blue\empty
\pdfadjustspacing=1
\noindent
\begingroup
\def\it{\textbullet}%
\def\sep{1ex}%
\begin{tabularx}{\linewidth}{@{}l@{ }X@{}}
  \it&\Blue{*pdfspec*} (version 1.3):\newline
    \link{http://partners.adobe.com/asn/developer/PDFS/TN/PDFSPEC.PDF}%
    \tabularnewline[\sep]
  \it&\Blue{*pdftex*}:
    \begingroup
      \settoheight{\dimen0}{\mbox{\^e}}%
      \settoheight{\dimen1}{\mbox{e}}%
      \addtolength{\dimen0}{-\dimen1}%
    (H\`an Th\rlap{\raise\dimen0\hbox{\'{}}}\^e Th\`anh):
    \endgroup
    \newline
    \link{http://www.tug.org/applications/pdftex/}\newline
    Win32: \link{ftp://ftp.ese-metz.fr/pub/TeX/win32-beta/}%
    \tabularnewline[\sep]
  \it&\Blue{*hyperref*} (Sebastian Rahtz):\hfill
    \link{ftp://ctan.tug.org/tex-archive/macros/latex/contrib/supported/hyperref/}%
    \newline
    Test versions:\newline
    \link{http://www.tug.org/applications/hyperref/hyperref.zip}
    \tabularnewline[\sep]
  \it&\Blue{*hypbmsec*} (Heiko Oberdiek):\hfill
    \link{ftp://ctan.tug.org/tex-archive/macros/latex/contrib/supported/oberdiek/}%
    \tabularnewline[\sep]
  \it&\Blue{*thumbpdf*} (Heiko Oberdiek):\newline
    \link{ftp://ctan.tug.org/tex-archive/macros/pdftex/thumbpdf/}%
\end{tabularx}
\endgroup
\end{smallpar}

%\SetNav{\NavFull\NavSep\NavPrev\NavSep\NavQuit}
\end{Nav}

\endinput


==> hyperref/navbook.tex <==
\newcommand{\bmaction}[3][0]{%
  \begingroup
    \pdfstringdef\x{#3}%
    \pdfoutline user {<</S /Named /N /#2>>} count #1 {\x}%
  \endgroup
}
\bmaction[-3]{NOP}{Navigation}
  \bmaction[2]{FullScreen}{Full-screen}
    \bmaction{PageOnly}{Page only}
    \bmaction{ShowThumbs}{Thumbnails}
  \bmaction[6]{NOP}{Selecting pages}
    \bmaction{PrevPage}{Previous page}
    \bmaction{NextPage}{Next page}
    \bmaction{GoBack}{Go back}
    \bmaction{GoForward}{Go forward}
    \bmaction{FirstPage}{First page}
    \bmaction{LastPage}{Last page}
  \bmaction[2]{GeneralInfo}{General document information}
    \bmaction{ShowHideMenuBar}{Menu bar}
    \bmaction{ShowHideToolBar}{Tool bar}

\endinput


==> hyperref/pdfextra.tex <==
\foilhead{Additional features of \abbr{pdf} format}
\noindent
Hyperref does not support all possibilities of *pdf* format, e.\,g.:
\begin{itemize}
  \let\Blue\empty
  \item \Blue{\Code{/CreationDate}} and \Blue{\Code{/ModDate}}.
  \item \Blue{Bookmarks} with \Blue{other functions}.
\end{itemize}
The following examples uses commands of \empty{*pdftex*}.

\subfoilhead{Bookmarks with other functions}
\begin{Nav}{\NavBookmarks\NavPage}

\begin{itemize}
  \item Menu functions of AcrobatReader, sound, video, \dots
  \item *pdftex* low level command:\\[1ex]
        \code[red]<\pdfoutline>\ \emph{\code<action>}\
        \code<count>\ \emph{\code[blue]<n>}\
        \code<{>\emph{\code<text>}\code<}>
        \begin{itemize}
          \item
            The absolute value of \emph{\code[blue]<n>}\ is the
            count of the direct subentries.
          \item
            If \emph{\code[blue]<n>}\ is negative, the
            subentries are closed.
        \end{itemize}
\end{itemize}


\subfoilhead{Link to external file}
\noindent
The *pdfspec* contains the possible actions on page 96.\\
At last a bookmark that points to that page:
\begingroup
  \edef\({\string(}
  \edef\){\string)}
\begin{verbatim}
$Blue(\pdfoutline)
  user {<<$Green(/S /GoToR /F $(pdfspec.pdf$) /D [95 /Fit])>>}
  count 0 {$empty(Description of actions)}
\end{verbatim}
\endgroup

\end{Nav}

\endinput


==> hyperref/pdfinfo.tex <==
\hypersetup!{%
  pdftitle!    = {PDF information and navigation elements},
  pdfsubject!  = {Slides for talk at EuroTeX'99 in Heidelberg},
  pdfkeywords! = {pdf, hyperref, bookmarks, thumbnails},
  pdfauthor!   = {\textcopyright\ Heiko Oberdiek},
  pdfcreator!  = {\LaTeX\ with package \flqq hyperref\frqq},
  pdfproducer! = {pdfeTeX-0.\the\pdftexversion\pdftexrevision},
}
\pdfinfo!{/CreationDate! (D:19990909000000-01'00')}

==> hyperref/psd.tex <==

\foilhead[-\baselineskip]{\cms{pdfstringdef}%
  \texorpdfstring{  converts \abbr{tex} to \abbr{pdf} strings}{}}

\noindent
Syntax: \Blue{\cms{pdfstringdef}}\Code{\{\emph{\cms{command}}\}%
    \{\emph{*tex* string}\}}

\begin{enumerate}
\item Selecting the encoding *PD1* or *PU*.
\item Redefinitions of many commands, so that they
      produce correct\\
      results or do not harm.
\item Expansion of the string.
\item Token checks and removal of forbidden tokens with 
      comprehensive\\ 
      warnings.
\end{enumerate}


\subfoilhead[-.5\baselineskip]{Redefinitions%
  \texorpdfstring{ by \cms{pdfstringdef}}{}}
\begin{itemize}
\item Redefinitions to get correct results, *eg*:
      \begin{itemize} 
      \item Glyph commands: \cms{\{}, \cms{\%}, \cms{space}, \cms{dots},
            \dots
      \item Logos: \cms{TeX}, \cms{LaTeX}, \cms{MF}, \dots
      \end{itemize}
\item Many tokens are removed silently, *eg*:
      \begin{itemize}
      \item *latex* commands: \cms{label}, \cms{index}, 
           \cms{textbf}, \dots
      \item Stomach tokens: curly group braces, \cms{relax} (\cms{protect}), 
            \dots
      \end{itemize}
\item The behaviour of \cms{xspace} is simulated.
\end{itemize}

\endinput


==> hyperref/replace.tex <==
\foilhead{Replacement methods}

\begin{itemize}
%\item \code[blue]<\texorpdfstring>\ provides an alternative.
\item \Blue{\cms{texorpdfstring}} choices one of its arguments:\\
      a *tex* or a *pdf* string.
\item \code[blue]<\pdfstringdefPreHook>\ is a place for redefining commands.\\
      Additions are made by \code[blue]<\pdfstringdefDisableCommands>.
\item Package \Blue{*hypbmsec*} extends the \code<\section>\ commands.
\end{itemize}


\subfoilhead{\cms{texorpdfstring} method}
\noindent
Syntax: \Red{\cms{texorpdfstring}}%
        \Green{\Code{\{*tex* string\}}}%
        \Blue{\Code{\{*pdf* string\}}}

\noindent
Example:

\noindent
  \cms{section}\Code{\{}\Red{\cms{texorpdfstring}}%
  %\Code{\emph{\%}}%
  \Green{\Code{\{H\$\_2\$O\}}}%
  %\Code{\emph{\%}}%
  \Blue{\Code{\{Water\}}}%
  %\Code{\emph{\%}}%
  \Code{\}}


\subfoilhead[-1\baselineskip]{Hook for private macro redefinitions}

\begin{itemize}
\item \Red{\cms{pdfstringdefPreHook}} is called, before expanding the string.
\item \Red{\cms{pdfstringdefDisableCommands}} adds user redefinitions to\\
      \cms{pdfstringdefPreHook}

  \Blue{\cms{pdfstringdefDisableCommands}}\Code{\{\commentchar}\\
  *ind*\cms{renewcommand}\Code{\{\cms{textcolor}\}[1]\{\#1\}\commentchar}\\
  *ind*\cms{renewcommand}\Code{\{\cms{url}\}}\Code{\{}\empty{\cms{pdfstringdefwarn}}%
    \Code{\{\cms{url}\}}\Code{\}\commentchar}\\
  *ind*\cms{let}\cms{textcolor}\cms{@gobble}\\
  \Code{\}}
\item \Red{\cms{pdfstringdefwarn}} prints a warning message.
\end{itemize}


\subfoilhead[-\baselineskip]{Package \Package{hypbmsec}}

\begin{itemize}
\item The syntax of \cms{section} commands is extended:
      \begin{itemize}
      \item Second optional bookmark argument.
      \item Bookmark in parentheses.
      \end{itemize}
\item Syntax:
  \def\txt{\Blue{\textsl{text}}}%
  \def\toc{\Green{\textsl{toc/head}}}%
  \def\out{\Red{\textsl{bookmark}}}%
  \settowidth{\dimen0}{\toc}%
  \settowidth{\dimen1}{\out}%
  \addtolength{\dimen1}{-\dimen0}%
  \setlength{\dimen1}{.5\dimen1}%
  \edef\toc{\noexpand\Green{\noexpand\textsl{toc%
    \noexpand\hspace{\the\dimen1}/\noexpand\hspace{\the\dimen1}head}}}%
  \settowidth{\dimen0}{\textbf{]\{}}%
  \settowidth{\dimen1}{ = }%
  \addtolength{\dimen0}{-\dimen1}%
  \setlength{\dimen0}{-.5\dimen0}%
  \edef\xsp{\noexpand\hspace{\the\dimen0}}%
  \def\({\textbf{(}\,}%
  \def\){\,\textbf{)}}%
  \def\[{\textbf{[}\,}%
  \def\]{\,\textbf{]}}%
  \def\{{\textbf{\orgbraceleft}\,}%
  \def\}{\,\textbf{\orgbraceright}}%
  \def\section{\cms{section}}%
  \def~{ = }%
  \begin{tabular}[t]{@{}l@{ }c@{}c@{}c@{}c@{}c@{}l@{}}
    \section&\{&\toc&~&\out&~&\txt\}\\
    \section&\[&\toc&~&\out&\]\,\{&\txt\}\\[1ex]
    \section&\[&\toc&\]\,\[&\out&\]\,\{&\txt\}\\[1ex]
    \section&\(&\out&\)\,\{&\toc&~&\txt\}\\
    \section&\[&\toc&\]\,\(&\out&\)\,\{&\txt\}\\
    \section&\(&\out&\)\,\[&\toc&\]\,\{&\txt\}\\
  \end{tabular}
\end{itemize}


\endinput

The next version of package *hypbmsec* will know the
option \Blue{\Option{startotoc}}:
The starred *sectioning* commands are included in the table
of contents and in the outline tree automatically.
For options \Blue{\Option{infix}} and \Blue{\Option{prefix}}
see \secref{sec:addcontentsline}.

\endinput


==> hyperref/strings.tex <==
\clearpage
\pdfbookmark[0]{Strings}{string}

\begingroup
\hypersetup{bookmarksopenlevel=2}

\subfoilhead[-\baselineskip]{\abbr{pdf} strings}

\begin{itemize}
\item Examples, where *pdf* strings are used:
      \begin{quote}
      Bookmark names, information dictionaries, text annotations
      \end{quote}
\item *pdf* strings follow the *postscript* rules:
      \begin{itemize}
      \item Delimited by parentheses: \Code{\Blue{(}This is a string\Blue{)}}
      \item Escape sequences for white space, \Blue{\cms{(}}, \Blue{\cms{)}},
            \Blue{\cms{}\cms{}};\\
            octal notation, *eg*: `\"a\"o\"u\ss' = 
            \Code{(}\Blue{\cms{344}\cms{366}\cms{374}\cms{337}}\Code{)}
      \end{itemize}
\item 
%      $\vcenter{\mbox{%
        \begin{tabular}[t]{@{}l@{ }l@{}}
          \Blue{*pdfdocencoding*}:&8bit, superset of *isolatin1*\\
          \Blue{*unicode*}:&16bit, *acroread* version $\ge$ 4\\
        \end{tabular}%
%      }}$ 
\end{itemize}


\clearpage
\pdfbookmark[1]{\abbr{tex} strings}{strings}

\subsubfoilhead[-.5\baselineskip]{Digestion of \abbr{tex}}

\begingroup
\newenvironment{organ}[2]{%
  \begin{minipage}[t]{\linewidth}%
    \vspace{#2}%
    \begin{tabbing}%
      \begin{tabular}{@{\textbullet\ }l@{}}
        \multicolumn{1}{@{}l@{}}{%
%          \phantom{\textbullet\ }%
          \textbf{\large\Blue{#1}}}\\[0.5ex]
}{
      \end{tabular}%
    \end{tabbing}%
  \end{minipage}%
}

\makeatletter
\let\fbox\@firstofone

\noindent
\fbox{%
\begin{organ}{Eyes}{0pt}
  Reading input lines\\
  Catcodes are set
\end{organ}}%
\hfill
\fbox{%
\begin{organ}{Mouth}{2\baselineskip}
  Forming tokens\\
  Expansion of macros
\end{organ}}%
\hfill
\fbox{%
\begin{organ}{Stomach}{4\baselineskip}
  Assignments\\
  Typesetting
\end{organ}}%

\endgroup


\subsubfoilhead[-.5\baselineskip]{Differences between mouth and stomach}

\noindent
\begin{tabular}{@{}lll@{}}
  &\Blue{\textbf{mouth}}&
   \Blue{\textbf{stomach}}\\[1ex]
``zero'':& \code<\empty>&\code<\relax>\\[0.5ex]
\code<{...}>:&parameter&group\\[0.5ex]
variable:&read and check&assignments\\[0.5ex]
fonts:&--&different fonts and encodings\\
&&ligatures\\[0.5ex]
Commands:&\code<\string>, \code<\number>&\code<\def>, \code<\hbox>, \code<$>\\
&\code<\if>, \code<\the>&\code<\begingroup>, \code<\special>
\end{tabular}


\subfoilhead[-.5\baselineskip]{\abbr{tex} into \abbr{pdf} strings}

\begin{itemize}
\item Reusing the argument of *sectioning* commands (*tex* string)\\
      for the bookmarks (*pdf* strings).
\item Limitations because of missing stomach digestion:
      \begin{itemize}
      \item No manipulation of boxes, no mathematics, no colors, \dots
      \item No change of fonts or encodings, no ligatures.
      \item No assignments (\cms{xspace} uses \cms{futurelet}).
      \item Unexpandable commands appear verbatim.
      \end{itemize}
\end{itemize}


\endgroup
\endinput

==> hyperref/summary.tex <==
\clearpage
\pdfbookmark[0]{End}{ende}

\subfoilhead[-1.5\baselineskip]{Summary}
\begin{itemize}
  \item \Red{General document information}:
    \begin{itemize}
      \item Options in \code[blue]<\hypersetup>\
            after \cms{usepackage}\Code{\{hyperref\}}.
    \end{itemize}
  \item \Red{Bookmarks}:
    \begin{itemize}
      \item Automatically added by \Blue{*hyperref*}.
      \item \Blue{Oral expansion}, no stomach commands (exceptions).
      \item Replacement methods: \code[blue]<\texorpdfstring>,\\
            \code[blue]<\pdfstringdefDisableCommands>, and
            \Blue{*hypbmsec*}.
      \item Low level commands only for special effects.
    \end{itemize}
  \item \Red{Thumbnails}: Automatically added by \Blue{*thumbpdf*}.
\end{itemize}


==> hyperref/thumb.tex <==

\foilhead{Thumbnails}
\begin{Nav}{\NavThumbnails\NavBookmarks}
\thisthumb{zurueck}
\begin{itemize}
  \item Another method for navigation:
    \begin{itemize}
      \item Choosing pages.
      \item Selecting page areas.
    \end{itemize}
  \item Contents:
    \begin{itemize}
      \item Thumbnail sketches of the pages.
      \item Other pictograms, symbols, \dots
      \item Empty.
    \end{itemize}
\end{itemize}


\subfoilhead{Adding thumbnails with \abbr{thumbpdf}}
\thisthumb{weiter}
\begingroup
  \centering
  \setlength{\unitlength}{1pt}
  % ca. max: 240mm x 100mm
  % ca. max: 700pt x 300pt
  \def\FileBox#1{\framebox(180,40){\Code{\vphantom{Hg}#1}}}
  \def\ProgBox[#1]#2{\makebox(160,60)[#1]{\vphantom{Hg}#2}}
  \def\Nummer[#1]#2{\makebox(20,60)[#1]{%
    \vphantom{Hg}%
    $\smash{%
      \textsf{\textcircled{\vphantom{\large#2}\Blue{\small#2}}}%
    }$%
  }}
  \def\Down{\makebox(0,0)[b]{\DOWNarrow}}%
  \def\Up{\makebox(0,0)[t]{\UParrow}}%
  \def\Right{\makebox(0,0)[r]{\RIGHTarrow}}%
  \begin{picture}(670,250)
    % Dateinamen
    \put(80,0){\FileBox{thumbdta.tex}}
    \put(80,100){\FileBox{\emph{jobname}.pdf}}
    \put(80,200){\FileBox{\emph{jobname}.tex}}
    \put(470,200){\FileBox{\Red{\emph{jobname}.pdf}}}
    % Pfeile
    \put(170,200){\line(0,-1){60}}
    \put(170,140){\Down}
    \put(170,100){\line(0,-1){60}}
    \put(170,40){\Down}
    \put(260,220){\line(1,0){210}}
    \put(470,220){\Right}
    \put(260,20){\line(1,0){105}}
    \put(365,20){\line(0,1){160}}
    \put(365,180){\Up}
    % Nummern
    \put(190,140){\Nummer[l]{1}}
    \put(190,40){\Nummer[l]{2}}
    \put(280,230){\Nummer[lb]{3}}
    % Programme
    \put(-10,40){\ProgBox[r]{*thumbpdf*}}
    \put(-10,140){\ProgBox[r]{*pdftex*}}
    \put(285,230){\ProgBox[b]{*pdftex*}}
    \put(285,150){\ProgBox[t]{\Code{thumbpdf.sty}}}
  \end{picture}
\endgroup

\subfoilhead[-\baselineskip]{How \abbr{thumbpdf} works}
\begingroup
  \centering
  \setlength{\unitlength}{1pt}
  % ca. max: 240mm x 100mm
  % ca. max: 700pt x 300pt
  \def\FileBox#1{\framebox(180,40){\Code{\vphantom{Hg}#1}}}
  \def\ProgBox[#1]#2{\makebox(160,60)[#1]{\vphantom{Hg}#2}}
  \def\Down{\makebox(0,0)[b]{\DOWNarrow}}%
  \def\Up{\makebox(0,0)[t]{\UParrow}}%
  \def\Right{\makebox(0,0)[r]{\RIGHTarrow}}%
  \def\Left{\makebox(0,0)[l]{\LEFTarrow}}%
  \begin{picture}(650,340)
    % Dateinamen
    \put(80,0){\FileBox{\Red{thumbdta.tex}}}
    \put(80,100){\FileBox{thumbdta.pdf}}
    \put(80,200){\FileBox{thumb\emph{???}.png}}
    \put(80,300){\FileBox{\emph{jobname}.pdf}}
    \put(420,150){\FileBox{thumbopt.tex}}
    \put(420,240){\FileBox{\emph{other images}}}
    % Pfeile
    \put(170,300){\line(0,-1){60}}
    \put(170,240){\Down}
    \put(170,200){\line(0,-1){60}}
    \put(170,140){\Down}
    \put(170,100){\line(0,-1){60}}
    \put(170,40){\Down}
    \put(360,170){\line(1,0){60}}
    \put(360,170){\Left}
    \put(510,240){\line(0,-1){50}}
    \put(510,190){\Down}
    % Programme
    \put(-10,40){\ProgBox[r]{\textsf{perl}}}
    \put(-10,140){\ProgBox[r]{*pdftex*}}
    \put(190,140){\ProgBox[l]{\Code{thumbpdf.tex}}}
    \put(-10,240){\ProgBox[r]{*gs*}}
  \end{picture}
\endgroup


\iffalse %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfoilhead{Thumbnails and *pdftex*}
\begin{itemize}
\item There is no direct support.
\item \code[blue]<\pdfimage> (*pdftex* versions below 0.14):
  \begin{itemize}
    \item[$+$] Image works as thumbnail.
    \item[$-$] No access to the image object number.
    \item[$-$] Image is on the page, must be
               moved out of the page.
  \end{itemize}
\item Low level commands
  \code[blue]<\pdfobj>\ and \code[blue]<\pdflastobj>\ are possible.
\end{itemize}

\clearpage
\pdfbookmark[1]{Project *thumbpdf*}{thumbpdf}
\subsubfoilhead[-\baselineskip]{Solution\texorpdfstring{ of project *thumbpdf*}{}}

\begin{enumerate}
  \item Generating the thumbnails \Blue{\file{thumb???.png}} by \Red{*gs*}.
  \item \Red{*pdftex*} runs \Red{\file{thumbpdf.tex}},
        thumbnails included by \code[blue]<\pdfimage>.
  \item The perl script \Red{\file{thumbpdf.pl}} reads
        \Blue{\file{thumbpdf.pdf}} and writes\\
        the object data in a *tex*
        readable form \Blue{\file{thumbdta.tex}}.
  \item Package \Red{\file{thumbpdf.sty}} inputs \Blue{\file{thumbdta.tex}},
        that contains the\\
        thumbnails as *pdf* objects (\code[blue]<\pdfobj>).
  \item The object numbers of the thumbnails (\code[blue]<\pdflastobj>)
        are added\\
        to the page attributes (\code[blue]<\pdfpageattr>).
\end{enumerate}


\subsubfoilhead[-.5\baselineskip]{User interface\texorpdfstring{ of *thumbpdf*}{}}

\begin{itemize}
  \def\master{\textsl{master}}%
  \item Command lines (\file{\master.tex} inputs \file{thumbpdf.sty}):
    \begin{enumerate}
      \item \texttt{\Blue{pdf}(\Blue{e},\Blue{la})\Blue{tex \master.tex}}
      \item \Blue{\texttt{thumbpdf \master}}
      \item \texttt{\Blue{pdf}(\Blue{e},\Blue{la})\Blue{tex \master.tex}}
    \end{enumerate}
  \item Another program than *gs* can be used:
    \begin{enumerate}
      \item[2a.] \Blue{\texttt{\textsl{ProgramThatGeneratesThumbnails} \master.pdf}}
      \item[2b.] \Blue{\texttt{thumbpdf}}
    \end{enumerate}
\end{itemize}

\fi %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subfoilhead[-\baselineskip]{Other images as thumbnails}

\begin{itemize}
\item With \Blue{\cms{thumb}} other images are declared as
      thumbnails in the\\ 
      optional file \Blue{\file{thumbopt.tex}}.
\item \Blue{\cms{thisthumb}} sets the thumbnail for the current page.
\end{itemize}
\begingroup
  \let\Red\Green
  \centering
  \begin{tabular}{@{}l@{\quad$\rightarrow$\quad}l@{}}
    \multicolumn{1}{@{}l}{\empty{\File{thumbopt.tex}}}&%
      \File{\emph{jobname}.tex}\\
    \hline
    \empty{\cms{thumb}}\Code{\{\Red{one}\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one}\}}\\
    \empty{\cms{thumb}}\Code{\{\Red{one.png}\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one.png}\}}\\
    \empty{\cms{thumb}}\Code{[\Red{two}]\{one\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{two}\}}\\
    \empty{\cms{thumb}}\Code{[\Red{one}]\{./extras/one.png\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one}\}}\\
  \end{tabular}
  \par
\endgroup

\end{Nav}

\endinput


==> hyperref/thumbopt.tex <==
\thumb[zurueck]{addthumb/thumb001.png}
\thumb[weiter]{addthumb/thumb002.png}


==> hyperref/title.tex <==
\pdfbookmark[0]{Beginning}{anfang}
\pdfbookmark[1]{Title}{title}

%\date{21st September 1999}% EuroTeX'99
\date{13rd October 1999}% first release for hyperref
\title{*pdf* information and navigation elements with
       hyperref, *pdftex*, and thumbpdf}
\author{Heiko Oberdiek\\\Email{oberdiek@ruf.uni-freiburg.de}}

\begingroup
  \LogoOff\aftergroup\LogoOn
  \Restriction{\unskip\centerline{\NavStart}}%
  \aftergroup\Restriction\aftergroup\empty
  \maketitle
  \begin{abstract}
    \noindent
    Additional possibilities for information and navigation through
    paper-less on-line documents that offer the PDF format.
  \end{abstract}
  \newpage
\endgroup

\subfoilhead{Subjects}
\begin{itemize}
\item General document information\hfill*hyperref*
\item Bookmarks/outlines\hfill*hyperref*
\item Thumbnails\hfill*thumbpdf*
\end{itemize}

\endinput


==> ts1/makets1.tex <==
\input fontinst.sty
\input textcomp.tex
\substitutesilent{n}{c}
\textcompfamily{ptm}{}
\textcompfamily{mbvx}{}
\textcompfamily{mntx}{}
\bye


==> ts1/october <==
Sebastian,

this reply took longer than expected, since the machine where I unpacked 
your package went down for about a week without prior announce.

First there are some omissions in the style file and/or the table:

\textblank    {'040}                               missing in the table
\textdivorced {'143} % divorced                    missing in both
\textdong     {'226} % Dong (currency of vietnam)  missing in both
\textpertenthousand {'230}                         missing in both
\textpilcrow  {'231}                               missing in both
\textbaht     {'232} % Baht (currency of thailand) missing in both


The 
\textshortequals 
should be taken from position {'055}, not as currently from {'177}:
The one at '177 is designed as a hanging hyphenchar, where '055 is non-
hanging (like usual hyphen).

I suggest to rename 
\textasciitilde {'176} to
\textlowtilde.
  In fact, the `ASCII tilde' is not defined in typographical terms, if it is 
high (like an accent) or low in its box. The dc fonts contain a high
`\textasciitilde'; the companion complement is by design low lying, 
therefore the suggested name \textlowtilde.

The 
\textbigcircle
is in fact that circle which is used by the \textcircled command. I 
therefore suggest to move the definition of \textcircled from OMSenc.def
to TS1. Here is the relevant snippet, adapted to TS1:

\DeclareTextCommand{\textcircled}{TS1}[1]{{%
   \ooalign{%
      \hfil \raise .07ex\hbox {\upshape#1}\hfil \crcr
      \char'117 % 
   }%
}}

Comment: Since the TS1 encoding provides oblique fonts (with oblique 
bigcircles!), the command \upshape can be removed.

The two tie accents are in fact meant to replace the definition of \t from
OMLenc.def (this is the only reference to OML in text mode). As a first step 
I suggest to use the `lowercase accent' everywhere, I'm just thinking on 
how to implement the choice of different accents according to the case of 
the accentee. This gives the following:

\DeclareTextAccent{\t}{TS1}{'032}

The definitions of 
\texttieaccentlowercase and \texttieaccentuppercase
can be dropped (both from the package and from the table).

[...]

Actually, here's what I'm suggesting for the accents designed for capital
letters:

There are commands like \capitalacute (you may want to add {text} to the 
names), defined in the following way:

%
% Acute accent for capitals
%
\DeclareTextAccentDefault{\capitalacute}{TS1}
\DeclareTextAccent{\capitalacute}{TS1}{'001}
%

This command can be used by the end user either directly or through 
definitions of the type

\DeclareTextCompositeCommand{\'}{T1}{X}{\capitalacute X}

None of the latter definitions should be provided by default, since they are 
probably rarely used.

Yours,
J"org Knappen.



==> xcolor/ChangeLog <==
Package `xcolor' by Dr. Uwe Kern
https://github.com/latex3/xcolor/issues

History
=======
2022/06/12 v2.14
* New features:
    - Load if it exists the code from LaTeX to define \mathcolor.
* Bugfixes (LaTeX Team)
    - Modify \XC@info to avoid spurious error from \colorlet{foo}{} issue #12
    - make \normalcolor, \colorbox, \fcolorbox \textcolor, \pagecolor, 
      \nopagecolor, \definecolor, \DefineNamedColor protected as in color.sty issue #17

2021/10/31 v2.13
* Bugfixes (LaTeX Team)
    - use \@backslashchar color rather than \string\color to
	generate internal csnames, to avoid relying on the
	current setting	of \escapechar
    - Declare dvisvgm option to match graphics and color packages.
	Make dvipdfm an alias for dvipdfmx
    - Modify \XC@info to avoid spurious text from \colorlet{foo}{.!50}

2016/05/11 v2.12
* New features:
    - \nopagecolor command as introduced in `color' v1.1a
      (example added to xcolor3.tex);
    - `luatex' driver option (code provided by DPC) to fix
      incompatibilities due to changes in new LuaTeX version.
* Bugfixes:
    - possible name conflict by \XC@ifxcase call;
    - incorrect internal \@hex@@Hex macro.

2007/01/21 v2.11
* New features:
    - color names `lime' and `teal' added to the set of predefined
      colors.
* Bugfix:
    - incorrect \XC@strip@comma call within `hyperref'-related options.

2006/11/28 v2.10
* New features:
    - `fixinclude' option prevents dvips from explicitly resetting
      current color to `black' before actually inserting an .eps file
      via \color{red}\includegraphics{foo}.
* Changes:
    - \colorbox and \fcolorbox made robust;
    - obsolete package option `pst' removed;
    - several changes to internal macros.
* Bugfixes:
    - incorrect processing of cmyk-type current color `.'.

2005/12/21 v2.09
* New features:
    - \definecolor and \color now accept space-separated color
      specifications, e.g., \color[rgb]{1 .5 0};
    - experimental `xcdraw' option extended to `pdftex' and `dvipdfm'
      drivers.
* Changes:
    - test file xcolor2.tex made compatible with recent changes in
      `pstricks';
    - test file xcolor3.tex extended;
    - driver test file xcolor4.tex extended to demonstrate the different
      frame drawing approaches;
    - more efficient implementation of driver-specific code.

2005/11/25 v2.08
* New features:
    - more flexibility for \fcolorbox arguments, e.g.,
      \fcolorbox[gray]{0.5}[wave]{580}{test};
    - \boxframe returns a frame of given dimensions;
    - new implementation of \f(rame)box and \fcolorbox as an extension
      of bug report latex/3655 to reduce pixel positioning errors in
      output devices;
    - `kernelfbox' option for those who prefer the previous \f(rame)box
      approach;
    - experimental `xcdraw' option uses PostScript commands to draw
      frames and color boxes in case of `dvips'.
* Bugfixes:
    - insufficient expression type detection within \colorlet;
    - wrong calculation in the unit interval reduction for negative
      integers (affecting color series and extended color expressions).

2005/11/12 v2.07
* New features:
    - color model `Hsb' allows to specify hue in degrees;
    - color model `tHsb' (`tuned Hsb') for user-defined hue
      configuration on color wheels;
    - easy generation of color harmonies derived from `Hsb' or `tHsb'
      color wheels, e.g., \color{red>wheel,1,12} yields an `analogous'
      color to `red' on a 12-spoke wheel;
    - additional 317 predefined color names according to rgb.txt, which
      is part of Unix/X11 distributions;
    - `svgnames' option extended by 4 colors taken from rgb.txt;
    - enhanced syntax for immediate conversion, e.g.,
      \definecolor{foo}{rgb:gray}{0.3} or \color[rgb:wave]{478};
    - \@ifundefinedcolor and \@ifundefinedmodel commands.
* Changes:
    - enhanced documentation;
    - several changes to internal macros.
* Bugfixes:
    - wrong calculation of color series components in some cases of
      negative step parameters.

2005/10/15 v2.06
* New features:
    - color model `wave' for (approximate) visualisation of light
      wavelengths, still somewhat experimental;
    - pseudo-model `ps' for colors defined by literal PostScript code
      in conjunction with `pstricks and `dvips'; an illustrative
      example for a gamma-correction approach is given in xcolor2.tex;
    - \substitutecolormodel command for replacement of missing or
      faulty driver-specific color models;
    - improved detection and handling of driver-specific color models;
    - `dvipdfmx' and `xetex' options to support these drivers;
    - generic driver test file xcolor4.tex.
* Changes:
    - \XC@strip@comma doesn't generate a trailing space anymore, which
      improves also the output of the `testcolors' environment.

2005/09/30 v2.05
* New features:
    - `testcolors' environment helps to test colors in different models,
      showing both the visual result and the model-specific parameters;
    - \extractcolorspecs puts model/color specification into two
      separate commands, as opposed to \extractcolorspec;
    - color names `pink' and `olive' added to the set of predefined
      colors.
* Bugfixes:
    - \definecolor{foo}{named}{bar} did not work in v2.04.

2005/09/23 v2.04
* New features:
    - preparation for usage of additional - driver-provided - color
      models;
    - `pstricks' users may now specify explicit color parameters within
      \psset and related commands, e.g., \psset{linecolor=[rgb]{1,0,0}};
      an illustrative example is given in xcolor2.tex.
* Changes:
    - color model names sanitized (i.e., turned to catcode 12)
      throughout the package;
    - \@namelet command deprecated because of name clash with
      `memoir' - please use \XC@let@cc instead
      (more \XC@let@.. commands are available as well);
    - simplified color conversion code by using the new \XC@ifxcase
      command;
    - some minor changes to internal macros.

2005/06/06 v2.03
* New features:
    - `fixpdftex' option loads `pdfcolmk' package in order to improve
      pdfTeX's color behaviour during page breaks.
* Changes:
    - some minor changes to internal macros.
* Bugfixes:
    - due to an incorrect \if statement within \XC@info, \colorlet
      caused trouble whenever its second argument started with two
      identical letters, e.g., \colorlet{rab}{oof};
    - argument processing of \XC@getcolor caused incompatibility with
      `msc' package;
    - `prologue' option caused incompatibility with `preview' package.

2005/03/24 v2.02
* New features:
    - \aftergroupedef command to reproduce \aftergroupdef's behaviour
      prior to v2.01;
    - xcolor's homepage www.ukern.de/tex/xcolor.html now provides also
      a ready-to-run TDS-compliant archive containing all required
      files.
* Changes:
    - \rowcolors and friends are solely enabled by the `table' option;
    - \@ifxempty changed back to more robust variant of v2.00.
* Bugfixes:
    - \psset{linecolor=\ifcase\foo red\or green\or blue\fi} did not work
      with `pstricks' (error introduced in v2.01).

2005/03/15 v2.01
* New features:
    - `prologue' option for comprehensive `named' color support in
      conjunction with `dvips': on-the-fly generation of PostScript
      prologue files with all color definitions, ready for dvips
      inclusion and/or post-processing with device-specific parameters
      (e.g., spot colors);
    - dvips prologue file xcolor.pro to support additional `named'
      colors;
    - \colorlet may now also be used to create named colors from
      arbitrary color expressions;
    - enhanced color definition syntax to allow for target-model
      specific color parameters, e.g.,
      \definecolor{red}{rgb/cmyk}{1,0,0/0,1,1,0}, facilitating the
      usage of tailor-made colors both for displays and printers;
    - `deferred definition' of colors: \preparecolor and
      \definecolors enable decoupling of color specification and control
      sequence generation, especially useful (= memory saving) for large
      lists of colors, of which only a few names are actually used;
    - `dvipsnames*' and `svgnames*' options to support deferred
      definition.
* Changes:
    - higher accuracy: most complement calculations are now exact for
      all 5-digit decimals;
    - \rangeRGB and similar variables may now be changed at any point
      in a document;
    - \aftergroupdef now performs only a first-level expansion of its
      code argument;
    - \XCfileversion and similar internal constants removed from .sty
      and .def files;
    - improved memory management (reduced generation of `multiletter
      control sequences' by \@ifundefined tests);
    - several internal macros improved and/or renamed.
* Bugfixes:
    - \XC@getcolor could cause unwanted spaces when \psset was used
      inside |pspicture| environments (`pstricks');
    - arithmetic overflow could happen when too many decimal digits
      were used within color parameters, e.g., as a result of `fp'
      calculations.

2004/07/04 v2.00
* New features:
    - extended functionality for color expressions: mix colors like a
      painter;
    - support for color blending: specify color mix expressions that
      are being blended with every displayed color;
    - \xglobal command for selective control of globality for color
      definitions, blends, and masks;
    - multiple step operations (e.g., \color{foo!!+++}) and access to
      individual members (e.g., \color{foo!![7]}) in color series;
    - \providecolor command to define only non-existent colors;
    - \definecolorset and \providecolorset commands to facilitate the
      construction of color sets with common underlying color model;
    - additional 147 predefined color names according to SVG 1.1
      specification;
    - `xpdfborder' key for setting the width of hyperlink borders in a
      more driver-independent way if `dvips' is used.
* Changes:
    - `color' package now completely integrated within `xcolor';
    - `override', `usenames', `nodvipsnames' options and \xdefinecolor
      command no longer needed;
    - `dvips' and `dvipsnames' options now independent of each other;
    - \tracingcolors's behaviour changed to make it more versatile and
      reduce log file size in standard cases;
    - \rdivide's syntax made more flexible (divide by numbers and/or
      dimensions);
    - code restructured, some internal commands renamed;
    - documentation rearranged and enhanced.
* Bugfixes:
    - \definecolor{foo}{named}{bar} did not work (error introduced in
      v1.11);
    - more robust behaviour of conditionals within `pstricks'
      key-values.

2004/05/09 v1.11
* New features:
    - switch \ifglobalcolors to control whether color definitions are
      global or local;
    - option `hyperref' provides color expression support for the
      border colors of hyperlinks, e.g.,
      \hypersetup{xurlbordercolor=red!50!yellow};
    - internal hooks \XC@bcolor, \XC@mcolor, and \XC@ecolor for
      additional code that has to be executed immediately before/after
      the current color is being displayed.
* Changes:
    - \XC@logcolor renamed to \XC@display, which is now the core color
      display command;
    - improved interface to `pstricks'.

2004/03/27 v1.10
* New features:
    - support for `named' model;
    - support for `dvips' colors
      (may now be used within color expressions);
    - internal representation of `ordinary' and `named' colors merged
      into unified data structure;
    - allow multiple `-' signs at the beginning of color expressions.
* Bugfixes:
    - commands like \color[named]{foo} caused errors when color masking
      or target model conversion were active;
    - incompatibility with `soul' package: commands \hl, \ul, etc.
      could yield unexpected results.
* Documentation:
    - added formula for general color expressions;
    - enhanced text and index;
    - removed dependence of index generation on local configuration
      file.

2004/02/16 v1.09
* New features:
    - color model `HTML', a 24-bit hexadecimal `RGB' variant;
      allows to specify colors like \color[HTML]{AFFE90};
    - color names `orange', `violet', `purple', and `brown' added to
      the set of predefined colors.
* New xcolor homepage: www.ukern.de/tex/xcolor.html
* Bugfix: \xdefinecolor sometimes did not normalise its parameters.
* Changes:
    - slight improvements of the documentation;
    - example file xcolor1.tex reorganised and abridged.

2004/02/04 v1.08
* New commands/features:
    - \selectcolormodel to change the target model within a document;
    - \adjustUCRBG to fine-tune undercolor-removal and
      black-generation during conversion to `cmyk'.
* Bugfix: color expressions did not work correctly in connection with
  active `!' character, e.g., in case of \usepackage[frenchb]{babel}.
* Code re-organisation:
    - \XC@xdefinecolor merged into \xdefinecolor, making the first
      command obsolete;
    - several internal commands improved/streamlined.

2004/01/20 v1.07
* New feature: support for color masking and color separation.
* New commands:
    - \rmultiply to multiply a dimension register by a real number;
    - \xcolorcmd to pass commands that are to be executed at the end
      of the package.
* Changes:
    - more consistent color handling: extended colors now always take
      precedence over standard colors;
    - several commands improved by using code from the LaTeX kernel.
* Documentation: some minor changes.
* Example files: additional `pstricks' examples (file xcolor2.tex).

2003/12/15 v1.06
* New feature: extended color expressions, allowing for cascaded mix
  operations, e.g., \color{red!30!green!40!blue}.
* Documentation: new section on color expressions.
* Bugfix: color series stepping did not work correctly within
  non-displaying commands like \extractcolorspec{foo!!+}
  (this bug was introduced in v1.05).
* Renamed commands: \ukfileversion and similar internal constants
  renamed to \XCfileversion etc.
* Removed commands: \ifXCpst and \ifXCtable made obsolete by a simple
  trick.

2003/11/21 v1.05
* Bugfixes:
    - package option `hideerrors' should now work as expected;
    - usage of `.' in the first color expression in a document caused
      an error due to incorrect initialisation.
* Code re-organisation: \extractcolorspec now uses \XC@splitcolor,
  making \XC@extract obsolete.

2003/11/09 v1.04
* New feature: easy access to current color within color expressions.
* New option: `override' to replace \definecolor by \xdefinecolor.
* New command: \tracingcolors for logging color-specific information.

2003/09/21 v1.03
* Change: bypass strange behaviour of some drivers.
* New feature: driver-sharing with `hyperref'.

2003/09/19 v1.02
* Change: \extractcolorspec and \colorlet now also accept color series
  as arguments.

2003/09/15 v1.01
* New feature: \definecolorseries and friends.
* Documentation: removed some `doc'-related side-effects.
* Code re-organisation: all calculation-related tools put to one place.
* Bugfixes:
    - \@rdivide: added \relax to fix problem with negative numerators;
    - \rowc@l@rs: replaced \@ifempty by \@ifxempty.

2003/09/09 v1.00
* First published release.

